Learning Smooth Humanoid Locomotion through Lipschitz-Constrained Policies

Reinforcement learning combined with sim-to-real transfer offers a general framework for developing locomotion controllers for legged robots. To facilitate successful deployment in the real world, smoothing techniques, such as low-pass filters and smoothness rewards, are often employed to develop policies with smooth behaviors. However, because these techniques are non-differentiable and usually require tedious tuning of a large set of hyperparameters, they tend to require extensive manual tuning for each robotic platform. To address this challenge and establish a general technique for enforcing smooth behaviors, we propose a simple and effective method that imposes a Lipschitz constraint on a learned policy, which we refer to as Lipschitz-Constrained Policies (LCP). We show that the Lipschitz constraint can be implemented in the form of a gradient penalty, which provides a differentiable objective that can be easily incorporated with automatic differentiation frameworks. We demonstrate that LCP effectively replaces the need for smoothing rewards or low-pass filters and can be easily integrated into training frameworks for many distinct humanoid robots. We extensively evaluate LCP in both simulation and real-world humanoid robots, producing smooth and robust locomotion controllers. All simulation and deployment code, along with complete checkpoints, is available on our project page: https://lipschitz-constrained-policy.github.io.

==> pre.tex <==
\newcommand{\half}{\ensuremath{\frac{1}{2}}}

\newcommand{\mnorm}[1]{\left\| #1 \right\|}

%bold-face vectors: maybe they're clearer
\newcommand{\mvec}[1]{\boldsymbol{#1}}
\newcommand{\mvecd}[1]{\dot{\boldsymbol{#1}}}
\newcommand{\mvecdd}[1]{\ddot{\boldsymbol{#1}}}

%matrices: (MATrix SYMbol)
\newcommand{\matSym}[1]{\boldsymbol{#1}}

\newcommand{\variance}[1]{\text{var} \left( #1 \right)} %variance of {.}

\newcommand{\grav}{\mvec{g}} %gravity vector

\newcommand{\mmat}[1]{\begin{bmatrix} #1 \end{bmatrix} }

\newcommand{\msum}[3]{\displaystyle\sum\limits_{#1}^{#2} {#3}}
\newcommand{\msumsmall}[3]{\sum\limits_{#1}^{#2} {#3}}
\newcommand{\mint}[4]{\ensuremath{\displaystyle\int\limits_{#1}^{#2} \! {#3} \, {#4} }}
\newcommand{\mpd} [2]{\frac{\partial #1}{\partial #2}} %partial differential
\newcommand{\mforall}{\; \forall \;}
\newcommand{\mlim}[1]{\underset{#1}\lim}
\newcommand{\mmax}[1]{\underset{#1}\max}
\newcommand{\mmin}[1]{\underset{#1}\min}
\newcommand{\mdeg}{^{\circ}}

\newcommand{\mrb}[1]{\left( #1 \right)} %enclose in round brackets
\newcommand{\msb}[1]{\left[ #1 \right]} %enclose in square brackets
\newcommand{\mcb}[1]{\left\{ #1 \right\}} %enclose in curly brackets
\newcommand{\mabs}[1]{\left| #1 \right|} %enclose in | . |

\newcommand{\littleO}[1]{{o}\mrb{#1}} %landau


\newcommand{\inv}[1]{#1^{-1}} %inverse

\newcommand{\dotp}[2]{#1^T#2} %dot product

\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
%\newcommand{\eqref}[1]{(\ref{#1})}

\newcommand{\realNums}{\ensuremath{\mathbb{R}}}
\newcommand{\crossMat}[1]{\ensuremath{\llbracket{#1}\rrbracket}}

\newcommand{\gravity}{\mvec{g}}

\newcommand{\expVal}[1]{\mathrm{E}\msb{#1}}


%newly added for the dynamics and control section:
\newcommand{\dtSample}{\Delta t}
\newcommand{\stateVec}{\mvec{\xi}}
\newcommand{\pos}{\ensuremath{\mvec{p}}}
\newcommand{\vel}{\ensuremath{\mvec{v}}}
\newcommand{\acc}{\ensuremath{\mvec{a}}}
\newcommand{\rotErr}{\ensuremath{\mvec{\delta}}}
\newcommand{\rot}{\ensuremath{\mvec{R}}}
\newcommand{\rotRef}{\ensuremath{\mvec{R}_\mathrm{ref}}}

\newcommand{\estStateVec}{\hat{\stateVec}}
\newcommand{\estPos}{\hat{\pos}}
\newcommand{\estVel}{\hat{\vel}}
\newcommand{\estAcc}{\hat{\acc}}
\newcommand{\estRotErr}{\hat{\rotErr}}
\newcommand{\estRot}{\hat{\rot}}
\newcommand{\estRotRef}{\ensuremath{\hat{\mvec{R}}_\mathrm{ref}}}

\newcommand{\skewSym}[1]{\ensuremath{\,S\!\mrb{#1}}}
\newcommand{\skewSymInv}[1]{\ensuremath{\,{v}\!\mrb{#1}}}


